Privacy-Preserving Public Information for Sequential Games

In settings with incomplete information, players can find it difficult to coordinate to find states with good social welfare. For example, in financial settings, if a collection of financial firms have limited information about each other's strategies, some large number of them may choose the same high-risk investment in hopes of high returns. While this might be acceptable in some cases, the economy can be hurt badly if many firms make investments in the same risky market segment and it fails. One reason why many firms might end up choosing the same segment is that they do not have information about other firms' investments (imperfect information may lead to `bad' game states). Directly reporting all players' investments, however, raises confidentiality concerns for both individuals and institutions. In this paper, we explore whether information about the game-state can be publicly announced in a manner that maintains the privacy of the actions of the players, and still suffices to deter players from reaching bad game-states. We show that in many games of interest, it is possible for players to avoid these bad states with the help of privacy-preserving, publicly-announced information. We model behavior of players in this imperfect information setting in two ways -- greedy and undominated strategic behaviours, and we prove guarantees on social welfare that certain kinds of privacy-preserving information can help attain. Furthermore, we design a counter with improved privacy guarantees under continual observation.

==> behavior-app.tex <==
\section{Formal Definitions of Behavior}\label{sec:behavior-app}



Since we consider game play with incomplete information, we need to
describe the strategy space of the players. We will analyze the game
play under two classes of strategies -- greedy and undominated
strategies. We assume that the value functions $\dvalo{r}$ for all $r$
are known to all players.
\begin{enumerate}
\item {\bf Greedy strategy:} Under the greedy strategy, a player
  chooses the action that maximizes her utility given the
  \emph{currently displayed (or announced) values of the
    counters}\footnote{Even with a \emph{future-dependent} utility
    function, the player will choose the resource that will maximize
    her utility function given the \emph{current counter} values
    during her turn (and not concern herself with what future players
    might choose).}. This means that when player $i$ gets her turn to
  play and say, $m_{i}(a_{1}, \cdots, a_{i-1})$ is $(\sused{i}{1},
  \cdots , \sused{i}{m})$, she picks the action $a_i = (\used{i}{1},
  \ldots, \used{i}{m})$ with largest $\sum_{r}\used{r}{i}
  \dval{\sused{i}{r}}{r}$\footnote{In the continuous case, she picks $a_i$
    such that $\sum_{r}\int_{\sused{i}{r}}^{\sused{i}{r} + \ract{i}{r}}
    \val{z}{r}dz)$.}. Such a player has no outside information or belief
  about the game or the types and the strategies of the other players.
%\item {\bf Approximately Greedy strategy:} Under some approximately
%  greedy strategy, we assume that each player $i$ is playing greedily
%  according to some \emph{reasonable belief} $\hat{\sused{i}{r}}$ about
%  each resource $r$'s use, which is at least as accurate in
%  expectation as the signal, which underestimates the count of $r$
%  with , that is, for all $i, r$, and for all correct values
%  $\used{i}{r}$, $\exp{|\hat{\sused{i}{r}} - \used{i}{r}|} \leq
%  \exp{|\sused{i}{r}- \used{i}{r}|}$ and $\prob[\hat{\sused{i}{r}} <
%  \used{i}{r} ] \geq \frac{1}{2}$.
\item {\bf Undominated Strategy(UD):} A player is allowed to play
  \emph{any} undominated strategy $a_i$ with respect to the
  announcements $\ssig{i}$, $i$'s signal.  A strategy $a_i$ is
  \emph{dominated} with respect to $m_i$ if there is some $a'_i$ for
  which $u_i(a'_i, a_{-i})>u_i(a_i, a_{-i})$ for all $a_{-i}$ which
  could cause $\ssig{i}$ with positive probability. If no such $a'_i$
  exists, $a_i$ is said to be undominated with respect to the signal
  $\ssig{i}$\footnote{ Note that, for arbitrary signaling mechanisms,
    undominated strategies are guaranteed to exist. For example, the
    greedy strategy with respect to the correct counts is always
    undominated, though players may not be able to implement this
    strategy; if the signalling mechanism has nonzero probability of
    outputting the correct counts, the greedy strategy with respect to
    the signals is undominated; if the mechanism has nonzero
    probability of outputting something with arbitrarily large error,
    then no strategy is undominated; in general, there may be a large
    class of undominated strategies and it is never empty.}. For
  instance, in a resource sharing game with an $(\alpha, \beta,
  0)$-accurate counter vector, picking resource $r$ for $i$ is
  dominated if there exists some resource $r'$ that $i$ has access to
  such that $\dval{\sused{i}{r'}/\alpha - \beta}{r'} >
  \dval{\alpha\sused{i}{r} + \beta}{r}$ and undominated otherwise.
\end{enumerate}


==> related.tex <==
\section{Related Work}\label{section:rw}
A great deal of work has been done at the intersection of mechanism
design and privacy; Pai and Roth~\citep{Pairoth13} have an extensive
survey. While the survey exhaustively covers the research work at the
intersection of the two areas, we list here a few key connections. One
line of work has employed techniques from differential privacy to
design incentive compatible mechanisms (for e.g.,
\citep{McSherry:2007, NST:2012}). More recently, differential privacy
has been considered as a constraint, and incentive compatible
mechanisms that satisfy this constraint while optimizing an objective
function have been designed \citep{Huang:2012, Xiao:2013}. In other
work, the utility function of agents have been redesigned to
incorporate privacy concerns, and mechanisms for the redesigned
utility functions have been constructed~\citep{Chen:2013, Ghosh:2011,
  Roth:2012, Katrina:2012, Fleischer:2012, NOS:2012}.

Our work is similar to some of the previous work in that it considers
maintaining differential privacy to be a constraint. The focus of our
work however is on \emph{how useful information can be provided to
  players in games of imperfect information} to help achieve a good
social objective while respecting the privacy constraint of the
players. The work of \citet{Kearns:2012} is close in spirit to
ours. \citet{Kearns:2012} consider a game where players have
incomplete information, and provide a mechanism that helps implement
an equilibrium by collecting the information from the players and
providing them suggestions on what actions to take. The mechanism is
designed so that it is incentive compatible for the players to
participate in the mechanism, and to follow its suggestions. Several
later papers \citep{congestionrogersR13, hsuwalrasian13} privately
compute approximate equillibria in different settings.

Our work which studies the ability of players to coordinate in cut
games, unrelated machine scheduling, and cost-sharing is inspired by
work of \citet{Leme:2012}. Their work focuses on the improvement in
social welfare of equilibria in the \emph{sequential} versus the
\emph{simultaneous} versions of certain games. We ask a related
question: when we consider sequential versions of games, and only
\emph{private, approximate information about the state of play} is
given to players, how much worse can social welfare be?

As mentioned in the introduction, one class of player behavior under
which we analyze the games is \emph{greedy}. Our analysis of greedy
behavior is in part inspired by the work of~\citet{balcan2009}, who
study best response dynamics with respect to noisy cost functions for
potential games. They ask: if players begin at some initial state, how
much can the social welfare degrade after a sequence of best-response
moves made with respect to noisy or slightly perturbed costs?  A
notable distinction between their setting and ours, however, is that
the noisy estimates we consider (and that differentially-private
counters provide) are \emph{estimates of state, not value}, and may
for natural value curves be quite far from correct in terms of the
{\em values} of the actions~\footnote{Having a `good' estimate for $x$
  does not necessarily imply a `good' estimate of $v(x)$ for many
  natural value curves $v(\cdot)$.}.
%\jmcomment{Do we want to talk about which games they
%  study? There's a lot of overlap..}% They show the Price of
%Uncertainty for market-sharing games is $\theta(\log(n))$, and that
%set-cover games' PoU are quite sensitive to the magnitude of the
%noise.

In a later section of this paper, we consider the case where players'
utilities depend on the actions of all other players. These games are
a generalization of market-sharing games\footnote{In the case of
  market-sharing, a market $r$ has a fixed value $v_r$, which is
  shared equally amongst players who service the market; we present a
  generalization of these games. Players can fractionally service
  markets, and for the restrictions on collections of markets can be
  arbitrary rather than budgetary.}. Previous
work~\citep{Goemans:2004} shows the Price of Anarchy of market-sharing
is 2, that players selecting $\beta$-approximately greedily in a
single round of best-response dynamics achieve a competitive ratio of
$\Theta((\beta + 1)\log(n))$. Market-sharing games are a special case
of congestion games, whose price of anarchy has been studied
extensively~\citep{christodoulou2005linear,christodoulou2005finite,
  roughgarden2004bounding, roughgarden2003price, suri2007selfish}, and
where greedy strategies have been shown to have constant competitive
ratio in special cases ~\citep{suri2007selfish, awerbuch1995load}.





